The strongly coupled $E_8\times E_8$ heterotic string: Geometry $\&$ Phenomenology

Working within the context of the strongly coupled $E_8\times E_8$ heterotic string theory, we analyze the $B-L$ MSSM, a realistic supersymmetric extension of the Standard Model, from both a low-energy phenomenology and high-energy string perspective. From a formal point of view, we examine different constructions of string vacua, which satisfy a series of theoretical and phenomenological constraints. Such vacua configurations are anomaly-free, preserve $N = 1$ SUSY at the compactification scale and yield the correct value for the $SO(10)$ unification scale and gauge coupling in the visible particle sector. Furthermore, we analyze a possible SUSY-breaking mechanism for the type of vacua we construct, via gaugino condensation in the hidden sector. In an attempt to connect these findings to experiment, we study the prospects of detecting the $B-L$ MSSM at the LHC in the near future. Within this specific context, we show that R-parity violating decays of supersymmetric particles could be amenable to direct detection at the ATLAS and CMS detectors. Detection of these processes would not only be an explicit indication of "Beyond the Standard Model" physics, but would also hint strongly at the existence of $N=1$ SUSY with spontaneously broken R-parity.

==> citations.tex <==
%\cite{Braun:2005bw}
\bibitem{Braun:2005bw}
V.~Braun, Y.~H.~He, B.~A.~Ovrut and T.~Pantev,
%``A Standard model from the E(8) x E(8) heterotic superstring,''
JHEP \textbf{06}, 039 (2005)
doi:10.1088/1126-6708/2005/06/039
[arXiv:hep-th/0502155 [hep-th]].
%134 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Braun:2005zv}
\bibitem{Braun:2005zv}
V.~Braun, Y.~H.~He, B.~A.~Ovrut and T.~Pantev,
%``Vector bundle extensions, sheaf cohomology, and the heterotic standard model,''
Adv. Theor. Math. Phys. \textbf{10}, no.4, 525-589 (2006)
doi:10.4310/ATMP.2006.v10.n4.a3
[arXiv:hep-th/0505041 [hep-th]].
%82 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Braun:2005nv}
\bibitem{Braun:2005nv}
V.~Braun, Y.~H.~He, B.~A.~Ovrut and T.~Pantev,
%``The Exact MSSM spectrum from string theory,''
JHEP \textbf{05}, 043 (2006)
doi:10.1088/1126-6708/2006/05/043
[arXiv:hep-th/0512177 [hep-th]].
%267 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Marshall:2014kea}
\bibitem{Marshall:2014kea}
Z.~Marshall, B.~A.~Ovrut, A.~Purves and S.~Spinner,
%``Spontaneous $R$-Parity Breaking, Stop LSP Decays and the Neutrino Mass Hierarchy,''
Phys. Lett. B \textbf{732}, 325-329 (2014)
doi:10.1016/j.physletb.2014.03.052
[arXiv:1401.7989 [hep-ph]].
%37 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Marshall:2014cwa}
\bibitem{Marshall:2014cwa}
Z.~Marshall, B.~A.~Ovrut, A.~Purves and S.~Spinner,
%``LSP Squark Decays at the LHC and the Neutrino Mass Hierarchy,''
Phys. Rev. D \textbf{90}, no.1, 015034 (2014)
doi:10.1103/PhysRevD.90.015034
[arXiv:1402.5434 [hep-ph]].
%32 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Dumitru:2018jyb}
\bibitem{Dumitru:2018jyb}
S.~Dumitru, B.~A.~Ovrut and A.~Purves,
%``The $R$-parity Violating Decays of Charginos and Neutralinos in the B-L MSSM,''
JHEP \textbf{02}, 124 (2019)
doi:10.1007/JHEP02(2019)124
[arXiv:1810.11035 [hep-ph]].
%12 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Dumitru:2018nct}
\bibitem{Dumitru:2018nct}
S.~Dumitru, B.~A.~Ovrut and A.~Purves,
%``$R$-parity Violating Decays of Wino Chargino and Wino Neutralino LSPs and NLSPs at the LHC,''
JHEP \textbf{06}, 100 (2019)
doi:10.1007/JHEP06(2019)100
[arXiv:1811.05581 [hep-ph]].
%11 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Dumitru:2019cgf}
\bibitem{Dumitru:2019cgf}
S.~Dumitru, C.~Herwig and B.~A.~Ovrut,
%``$R$-parity Violating Decays of Bino Neutralino LSPs at the LHC,''
JHEP \textbf{12}, 042 (2019)
doi:10.1007/JHEP12(2019)042
[arXiv:1906.03174 [hep-ph]].
%5 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Horava:1995qa}
\bibitem{Horava:1995qa}
P.~Horava and E.~Witten,
%``Heterotic and type I string dynamics from eleven-dimensions,''
Nucl. Phys. B \textbf{460}, 506-524 (1996)
doi:10.1016/0550-3213(95)00621-4
[arXiv:hep-th/9510209 [hep-th]].
%2520 citations counted in INSPIRE as of 17 May 2022

%\cite{Horava:1996ma}
\bibitem{Horava:1996ma}
P.~Horava and E.~Witten,
%``Eleven-dimensional supergravity on a manifold with boundary,''
Nucl. Phys. B \textbf{475}, 94-114 (1996)
doi:10.1016/0550-3213(96)00308-2
[arXiv:hep-th/9603142 [hep-th]].
%1871 citations counted in INSPIRE as of 19 May 2022

%\cite{Lukas:1998yy}
\bibitem{Lukas:1998yy}
A.~Lukas, B.~A.~Ovrut, K.~S.~Stelle and D.~Waldram,
%``The Universe as a domain wall,''
Phys. Rev. D \textbf{59}, 086001 (1999)
doi:10.1103/PhysRevD.59.086001
[arXiv:hep-th/9803235 [hep-th]].
%667 citations counted in INSPIRE as of 11 May 2022

%\cite{Lukas:1998tt}
\bibitem{Lukas:1998tt}
A.~Lukas, B.~A.~Ovrut, K.~S.~Stelle and D.~Waldram,
%``Heterotic M theory in five-dimensions,''
Nucl. Phys. B \textbf{552}, 246-290 (1999)
doi:10.1016/S0550-3213(99)00196-0
[arXiv:hep-th/9806051 [hep-th]].
%424 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Lukas:1997fg}
\bibitem{Lukas:1997fg}
A.~Lukas, B.~A.~Ovrut and D.~Waldram,
%``On the four-dimensional effective action of strongly coupled heterotic string theory,''
Nucl. Phys. B \textbf{532}, 43-82 (1998)
doi:10.1016/S0550-3213(98)00463-5
[arXiv:hep-th/9710208 [hep-th]].
%271 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Lukas:1998hk}
\bibitem{Lukas:1998hk}
A.~Lukas, B.~A.~Ovrut and D.~Waldram,
%``Nonstandard embedding and five-branes in heterotic M theory,''
Phys. Rev. D \textbf{59}, 106005 (1999)
doi:10.1103/PhysRevD.59.106005
[arXiv:hep-th/9808101 [hep-th]].
%147 citations counted in INSPIRE as of 14 May 2022

%\cite{Ovrut:2018qog}
\bibitem{Ovrut:2018qog}
B.~A.~Ovrut,
%``Vacuum Constraints for Realistic Strongly Coupled Heterotic M-Theories,''
Symmetry \textbf{10}, no.12, 723 (2018)
doi:10.3390/sym10120723
[arXiv:1811.08892 [hep-th]].
%8 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Ashmore:2020ocb}
\bibitem{Ashmore:2020ocb}
A.~Ashmore, S.~Dumitru and B.~A.~Ovrut,
%``Line Bundle Hidden Sectors for Strongly Coupled Heterotic Standard Models,''
Fortsch. Phys. \textbf{69}, no.7, 2100052 (2021)
doi:10.1002/prop.202100052
[arXiv:2003.05455 [hep-th]].
%7 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Ashmore:2021xdm}
\bibitem{Ashmore:2021xdm}
A.~Ashmore, S.~Dumitru and B.~A.~Ovrut,
%``Hidden Sectors from Multiple Line Bundles for the $B-L$ MSSM,''
[arXiv:2106.09087 [hep-th]].
%3 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Braun:2004xv}
\bibitem{Braun:2004xv}
V.~Braun, B.~A.~Ovrut, T.~Pantev and R.~Reinbacher,
%``Elliptic Calabi-Yau threefolds with Z(3) x Z(3) Wilson lines,''
JHEP \textbf{12}, 062 (2004)
doi:10.1088/1126-6708/2004/12/062
[arXiv:hep-th/0410055 [hep-th]].
%74 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Gomez:2005ii}
\bibitem{Gomez:2005ii}
T.~L.~Gomez, S.~Lukic and I.~Sols,
%``Constraining the Kahler moduli in the heterotic standard model,''
Commun. Math. Phys. \textbf{276}, 1-21 (2007)
doi:10.1007/s00220-007-0338-8
[arXiv:hep-th/0512205 [hep-th]].
%23 citations counted in INSPIRE as of 03 May 2022

%\cite{Braun:2006ae}
\bibitem{Braun:2006ae}
V.~Braun, Y.~H.~He and B.~A.~Ovrut,
%``Stability of the minimal heterotic standard model bundle,''
JHEP \textbf{06}, 032 (2006)
doi:10.1088/1126-6708/2006/06/032
[arXiv:hep-th/0602073 [hep-th]].
%40 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Deen:2016vyh}
\bibitem{Deen:2016vyh}
R.~Deen, B.~A.~Ovrut and A.~Purves,
%``The minimal SUSY B \ensuremath{-} L model: simultaneous Wilson lines and string thresholds,''
JHEP \textbf{07}, 043 (2016)
doi:10.1007/JHEP07(2016)043
[arXiv:1604.08588 [hep-ph]].
%14 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Ambroso:2009jd}
\bibitem{Ambroso:2009jd}
M.~Ambroso and B.~Ovrut,
%``The B-L/Electroweak Hierarchy in Heterotic String and M-Theory,''
JHEP \textbf{10}, 011 (2009)
doi:10.1088/1126-6708/2009/10/011
[arXiv:0904.4509 [hep-th]].
%48 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Ovrut:2012wg}
\bibitem{Ovrut:2012wg}
B.~A.~Ovrut, A.~Purves and S.~Spinner,
%``Wilson Lines and a Canonical Basis of SU(4) Heterotic Standard Models,''
JHEP \textbf{11}, 026 (2012)
doi:10.1007/JHEP11(2012)026
[arXiv:1203.1325 [hep-th]].
%30 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Ovrut:2014rba}
\bibitem{Ovrut:2014rba}
B.~A.~Ovrut, A.~Purves and S.~Spinner,
%``A statistical analysis of the minimal SUSY B\textendash{}L theory,''
Mod. Phys. Lett. A \textbf{30}, no.18, 1550085 (2015)
doi:10.1142/S0217732315500856
[arXiv:1412.6103 [hep-ph]].
%24 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Ovrut:2015uea}
\bibitem{Ovrut:2015uea}
B.~A.~Ovrut, A.~Purves and S.~Spinner,
%``The minimal SUSY $B − L$ model: from the unification scale to the LHC,''
JHEP \textbf{06}, 182 (2015)
doi:10.1007/JHEP06(2015)182
[arXiv:1503.01473 [hep-ph]].
%24 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Barger:2008wn}
\bibitem{Barger:2008wn}
V.~Barger, P.~Fileviez Perez and S.~Spinner,
%``Minimal gauged U(1)(B-L) model with spontaneous R-parity violation,''
Phys. Rev. Lett. \textbf{102}, 181802 (2009)
doi:10.1103/PhysRevLett.102.181802
[arXiv:0812.3661 [hep-ph]].
%136 citations counted in INSPIRE as of 20 May 2022

%\cite{FileviezPerez:2009gr}
\bibitem{FileviezPerez:2009gr}
P.~Fileviez Perez and S.~Spinner,
%``Spontaneous R-Parity Breaking in SUSY Models,''
Phys. Rev. D \textbf{80}, 015004 (2009)
doi:10.1103/PhysRevD.80.015004
[arXiv:0904.2213 [hep-ph]].
%44 citations counted in INSPIRE as of 10 May 2022

%\cite{FileviezPerez:2012mj}
\bibitem{FileviezPerez:2012mj}
P.~Fileviez Perez and S.~Spinner,
%``The Minimal Theory for R-parity Violation at the LHC,''
JHEP \textbf{04}, 118 (2012)
doi:10.1007/JHEP04(2012)118
[arXiv:1201.5923 [hep-ph]].
%70 citations counted in INSPIRE as of 10 May 2022

%\cite{Donagi:1998xe}
\bibitem{Donagi:1998xe}
R.~Donagi, A.~Lukas, B.~A.~Ovrut and D.~Waldram,
%``Nonperturbative vacua and particle physics in M theory,''
JHEP \textbf{05}, 018 (1999)
doi:10.1088/1126-6708/1999/05/018
[arXiv:hep-th/9811168 [hep-th]].
%106 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Donagi:1999gc}
\bibitem{Donagi:1999gc}
R.~Donagi, A.~Lukas, B.~A.~Ovrut and D.~Waldram,
%``Holomorphic vector bundles and nonperturbative vacua in M theory,''
JHEP \textbf{06}, 034 (1999)
doi:10.1088/1126-6708/1999/06/034
[arXiv:hep-th/9901009 [hep-th]].
%132 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Lukas:1999kt}
\bibitem{Lukas:1999kt}
A.~Lukas, B.~A.~Ovrut and D.~Waldram,
%``Five-branes and supersymmetry breaking in M theory,''
JHEP \textbf{04}, 009 (1999)
doi:10.1088/1126-6708/1999/04/009
[arXiv:hep-th/9901017 [hep-th]].
%91 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Brandle:2003uya}
\bibitem{Brandle:2003uya}
M.~Brandle,
%``Aspects of branes in (heterotic) M-theory,''
%3 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Anderson:2009nt}
\bibitem{Anderson:2009nt}
L.~B.~Anderson, J.~Gray, A.~Lukas and B.~Ovrut,
%``Stability Walls in Heterotic Theories,''
JHEP \textbf{09}, 026 (2009)
doi:10.1088/1126-6708/2009/09/026
[arXiv:0905.1748 [hep-th]].
%81 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Weigand:2006yj}
\bibitem{Weigand:2006yj}
T.~Weigand,
%``Compactifications of the heterotic string with unitary bundles,''
Fortsch. Phys. \textbf{54}, 963-1077 (2006)
doi:10.1002/prop.200610327
%19 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Moore:2000fs}
\bibitem{Moore:2000fs}
G.~W.~Moore, G.~Peradze and N.~Saulina,
%``Instabilities in heterotic M theory induced by open membrane instantons,''
Nucl. Phys. B \textbf{607}, 117-154 (2001)
doi:10.1016/S0550-3213(01)00155-9
[arXiv:hep-th/0012104 [hep-th]].
%73 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Banks:1996ss}
\bibitem{Banks:1996ss}
T.~Banks and M.~Dine,
%``Couplings and scales in strongly coupled heterotic string theory,''
Nucl. Phys. B \textbf{479}, 173-196 (1996)
doi:10.1016/0550-3213(96)00457-9
[arXiv:hep-th/9605136 [hep-th]].
%307 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Conrad:1997ww}
\bibitem{Conrad:1997ww}
J.~O.~Conrad,
%``Brane tensions and coupling constants from within M theory,''
Phys. Lett. B \textbf{421}, 119-124 (1998)
doi:10.1016/S0370-2693(97)01575-X
[arXiv:hep-th/9708031 [hep-th]].
%53 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Dienes:1996du}
\bibitem{Dienes:1996du}
K.~R.~Dienes,
%``String theory and the path to unification: A Review of recent developments,''
Phys. Rept. \textbf{287}, 447-525 (1997)
doi:10.1016/S0370-1573(97)00009-4
[arXiv:hep-th/9602045 [hep-th]].
%409 citations counted in INSPIRE as of 12 May 2022

%\cite{Bailin:2014nna}
\bibitem{Bailin:2014nna}
D.~Bailin and A.~Love,
%``Reduced modular symmetries of threshold corrections and gauge coupling unification,''
JHEP \textbf{04}, 002 (2015)
doi:10.1007/JHEP04(2015)002
[arXiv:1412.7327 [hep-th]].
%9 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Nilles:1998uy}
\bibitem{Nilles:1998uy}
H.~P.~Nilles,
%``On the Low-energy limit of string and M theory,''
[arXiv:hep-ph/0004064 [hep-ph]].
%32 citations counted in INSPIRE as of 13 May 2022

%\cite{Ovrut:2000qi}
\bibitem{Ovrut:2000qi}
B.~A.~Ovrut, T.~Pantev and J.~Park,
%``Small instanton transitions in heterotic M theory,''
JHEP \textbf{05}, 045 (2000)
doi:10.1088/1126-6708/2000/05/045
[arXiv:hep-th/0001133 [hep-th]].
%85 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Green:1984sg}
\bibitem{Green:1984sg}
M.~B.~Green and J.~H.~Schwarz,
%``Anomaly Cancellation in Supersymmetric D=10 Gauge Theory and Superstring Theory,''
Phys. Lett. B \textbf{149}, 117-122 (1984)
doi:10.1016/0370-2693(84)91565-X
%2942 citations counted in INSPIRE as of 19 May 2022

%\cite{Green:1987mn}
\bibitem{Green:1987mn}
M.~B.~Green, J.~H.~Schwarz and E.~Witten,
%``SUPERSTRING THEORY. VOL. 2: LOOP AMPLITUDES, ANOMALIES AND PHENOMENOLOGY,''
%254 citations counted in INSPIRE as of 05 May 2022

%\cite{Freedman:2012zz}
\bibitem{Freedman:2012zz}
D.~Z.~Freedman and A.~Van Proeyen,
%``Supergravity,''
%62 citations counted in INSPIRE as of 03 May 2022

%\cite{Blumenhagen:2005ga}
\bibitem{Blumenhagen:2005ga}
R.~Blumenhagen, G.~Honecker and T.~Weigand,
%``Loop-corrected compactifications of the heterotic string with line bundles,''
JHEP \textbf{06}, 020 (2005)
doi:10.1088/1126-6708/2005/06/020
[arXiv:hep-th/0504232 [hep-th]].
%189 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Anderson:2009sw}
\bibitem{Anderson:2009sw}
L.~B.~Anderson, J.~Gray, A.~Lukas and B.~Ovrut,
%``The Edge Of Supersymmetry: Stability Walls in Heterotic Theory,''
Phys. Lett. B \textbf{677}, 190-194 (2009)
doi:10.1016/j.physletb.2009.05.025
[arXiv:0903.5088 [hep-th]].
%57 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Dine:1986zy}
\bibitem{Dine:1986zy}
M.~Dine, N.~Seiberg, X.~G.~Wen and E.~Witten,
%``Nonperturbative Effects on the String World Sheet,''
Nucl. Phys. B \textbf{278}, 769-789 (1986)
doi:10.1016/0550-3213(86)90418-9
%432 citations counted in INSPIRE as of 28 Apr 2022

%\cite{Dine:1987xk}
\bibitem{Dine:1987xk}
M.~Dine, N.~Seiberg and E.~Witten,
%``Fayet-Iliopoulos Terms in String Theory,''
Nucl. Phys. B \textbf{289}, 589-598 (1987)
doi:10.1016/0550-3213(87)90395-6
%715 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Lukas:1999nh}
\bibitem{Lukas:1999nh}
A.~Lukas and K.~S.~Stelle,
%``Heterotic anomaly cancellation in five-dimensions,''
JHEP \textbf{01}, 010 (2000)
doi:10.1088/1126-6708/2000/01/010
[arXiv:hep-th/9911156 [hep-th]].
%82 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Wess:1992cp}
\bibitem{Wess:1992cp}
J.~Wess and J.~Bagger,
%``Supersymmetry and supergravity,''
%430 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Braun:2005ux}
\bibitem{Braun:2005ux}
V.~Braun, Y.~H.~He, B.~A.~Ovrut and T.~Pantev,
%``A Heterotic standard model,''
Phys. Lett. B \textbf{618}, 252-258 (2005)
doi:10.1016/j.physletb.2005.05.007
[arXiv:hep-th/0501070 [hep-th]].
%240 citations counted in INSPIRE as of 14 May 2022

%\cite{Braun:2013wr}
\bibitem{Braun:2013wr}
V.~Braun, Y.~H.~He and B.~A.~Ovrut,
%``Supersymmetric Hidden Sectors for Heterotic Standard Models,''
JHEP \textbf{09}, 008 (2013)
doi:10.1007/JHEP09(2013)008
[arXiv:1301.6767 [hep-th]].
%22 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Anderson:2010ty}
\bibitem{Anderson:2010ty}
L.~B.~Anderson, J.~Gray and B.~A.~Ovrut,
%``Transitions in the Web of Heterotic Vacua,''
Fortsch. Phys. \textbf{59}, 327-371 (2011)
doi:10.1002/prop.201000100
[arXiv:1012.3179 [hep-th]].
%24 citations counted in INSPIRE as of 25 Apr 2022

%\cite{0905.1748}
\bibitem{0905.1748}
L.~B.~Anderson, J.~Gray, A.~Lukas and B.~Ovrut,
%``Stability Walls in Heterotic Theories,''
JHEP \textbf{09}, 026 (2009)
doi:10.1088/1126-6708/2009/09/026
[arXiv:0905.1748 [hep-th]].
%81 citations counted in INSPIRE as of 29 Apr 2022

%\cite{1012.3179}
\bibitem{1012.3179}
L.~B.~Anderson, J.~Gray and B.~A.~Ovrut,
%``Transitions in the Web of Heterotic Vacua,''
Fortsch. Phys. \textbf{59}, 327-371 (2011)
doi:10.1002/prop.201000100
[arXiv:1012.3179 [hep-th]].
%24 citations counted in INSPIRE as of 25 Apr 2022

%\cite{1506.00879}
\bibitem{1506.00879}
S.~Groot Nibbelink, O.~Loukas, F.~Ruehle and P.~K.~S.~Vaudrevange,
%``Infinite number of MSSMs from heterotic line bundles?,''
Phys. Rev. D \textbf{92}, no.4, 046002 (2015)
doi:10.1103/PhysRevD.92.046002
[arXiv:1506.00879 [hep-th]].
%24 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Anderson:2012yf}
\bibitem{Anderson:2012yf}
L.~B.~Anderson, J.~Gray, A.~Lukas and E.~Palti,
%``Heterotic Line Bundle Standard Models,''
JHEP \textbf{06}, 113 (2012)
doi:10.1007/JHEP06(2012)113
[arXiv:1202.1757 [hep-th]].
%174 citations counted in INSPIRE as of 14 May 2022

%\cite{Nibbelink:2015ixa}
\bibitem{Nibbelink:2015ixa}
S.~Groot Nibbelink, O.~Loukas, F.~Ruehle and P.~K.~S.~Vaudrevange,
%``Infinite number of MSSMs from heterotic line bundles?,''
Phys. Rev. D \textbf{92}, no.4, 046002 (2015)
doi:10.1103/PhysRevD.92.046002
[arXiv:1506.00879 [hep-th]].
%24 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Nibbelink:2016wms}
\bibitem{Nibbelink:2016wms}
S.~Groot Nibbelin and F.~Ruehle,
%``Line bundle embeddings for heterotic theories,''
JHEP \textbf{04}, 186 (2016)
doi:10.1007/JHEP04(2016)186
[arXiv:1601.00676 [hep-th]].
%8 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Ashmore:2020wwv}
\bibitem{Ashmore:2020wwv}
A.~Ashmore, S.~Dumitru and B.~A.~Ovrut,
%``Explicit soft supersymmetry breaking in the heterotic M-theory B \ensuremath{-} L MSSM,''
JHEP \textbf{08}, 033 (2021)
doi:10.1007/JHEP08(2021)033
[arXiv:2012.11029 [hep-th]].
%5 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Feger:2012bs}
\bibitem{Feger:2012bs}
R.~Feger and T.~W.~Kephart,
%``LieART\textemdash{}A Mathematica application for Lie algebras and representation theory,''
Comput. Phys. Commun. \textbf{192}, 166-195 (2015)
doi:10.1016/j.cpc.2014.12.023
[arXiv:1206.6379 [math-ph]].
%152 citations counted in INSPIRE as of 12 May 2022

%\cite{Feger:2019tvk}
\bibitem{Feger:2019tvk}
R.~Feger, T.~W.~Kephart and R.~J.~Saskowski,
%``LieART 2.0 \textendash{} A Mathematica application for Lie Algebras and Representation Theory,''
Comput. Phys. Commun. \textbf{257}, 107490 (2020)
doi:10.1016/j.cpc.2020.107490
[arXiv:1912.10969 [hep-th]].
%46 citations counted in INSPIRE as of 17 May 2022

%\cite{Nibbelink:2007rd}
\bibitem{Nibbelink:2007rd}
S.~Groot Nibbelink, M.~Trapletti and M.~Walter,
%``Resolutions of C**n/Z(n) Orbifolds, their U(1) Bundles, and Applications to String Model Building,''
JHEP \textbf{03}, 035 (2007)
doi:10.1088/1126-6708/2007/03/035
[arXiv:hep-th/0701227 [hep-th]].
%64 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Dine:1985rz}
\bibitem{Dine:1985rz}
M.~Dine, R.~Rohm, N.~Seiberg and E.~Witten,
%``Gluino Condensation in Superstring Models,''
Phys. Lett. B \textbf{156}, 55-60 (1985)
doi:10.1016/0370-2693(85)91354-1
%955 citations counted in INSPIRE as of 19 May 2022

%\cite{Lukas:1997rb}
\bibitem{Lukas:1997rb}
A.~Lukas, B.~A.~Ovrut and D.~Waldram,
%``Gaugino condensation in M theory on s**1 / Z(2),''
Phys. Rev. D \textbf{57}, 7529-7538 (1998)
doi:10.1103/PhysRevD.57.7529
[arXiv:hep-th/9711197 [hep-th]].
%161 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Nilles:1998sx}
\bibitem{Nilles:1998sx}
H.~P.~Nilles, M.~Olechowski and M.~Yamaguchi,
%``Supersymmetry breakdown at a hidden wall,''
Nucl. Phys. B \textbf{530}, 43-72 (1998)
doi:10.1016/S0550-3213(98)00418-0
[arXiv:hep-th/9801030 [hep-th]].
%143 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Brandle:2001ts}
\bibitem{Brandle:2001ts}
M.~Brandle and A.~Lukas,
%``Five-branes in heterotic brane world theories,''
Phys. Rev. D \textbf{65}, 064024 (2002)
doi:10.1103/PhysRevD.65.064024
[arXiv:hep-th/0109173 [hep-th]].
%31 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Anderson:2010mh}
\bibitem{Anderson:2010mh}
L.~B.~Anderson, J.~Gray, A.~Lukas and B.~Ovrut,
%``Stabilizing the Complex Structure in Heterotic Calabi-Yau Vacua,''
JHEP \textbf{02}, 088 (2011)
doi:10.1007/JHEP02(2011)088
[arXiv:1010.0255 [hep-th]].
%84 citations counted in INSPIRE as of 14 May 2022

%\cite{Anderson:2011cza}
\bibitem{Anderson:2011cza}
L.~B.~Anderson, J.~Gray, A.~Lukas and B.~Ovrut,
%``Stabilizing All Geometric Moduli in Heterotic Calabi-Yau Vacua,''
Phys. Rev. D \textbf{83}, 106011 (2011)
doi:10.1103/PhysRevD.83.106011
[arXiv:1102.0011 [hep-th]].
%99 citations counted in INSPIRE as of 14 May 2022

%\cite{Anderson:2011ty}
\bibitem{Anderson:2011ty}
L.~B.~Anderson, J.~Gray, A.~Lukas and B.~Ovrut,
%``The Atiyah Class and Complex Structure Stabilization in Heterotic Calabi-Yau Compactifications,''
JHEP \textbf{10}, 032 (2011)
doi:10.1007/JHEP10(2011)032
[arXiv:1107.5076 [hep-th]].
%70 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Correia:2007sv}
\bibitem{Correia:2007sv}
F.~Paccetti Correia and M.~G.~Schmidt,
%``Moduli stabilization in heterotic M-theory,''
Nucl. Phys. B \textbf{797}, 243-267 (2008)
doi:10.1016/j.nuclphysb.2008.01.005
[arXiv:0708.3805 [hep-th]].
%24 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Yamatsu:2015npn}
\bibitem{Yamatsu:2015npn}
N.~Yamatsu,
%``Finite-Dimensional Lie Algebras and Their Representations for Unified Model Building,''
[arXiv:1511.08771 [hep-ph]].
%83 citations counted in INSPIRE as of 26 Apr 2022

%\cite{Soni:1983rm}
\bibitem{Soni:1983rm}
S.~K.~Soni and H.~A.~Weldon,
%``Analysis of the Supersymmetry Breaking Induced by N=1 Supergravity Theories,''
Phys. Lett. B \textbf{126}, 215-219 (1983)
doi:10.1016/0370-2693(83)90593-2
%378 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Kaplunovsky:1993rd}
\bibitem{Kaplunovsky:1993rd}
V.~S.~Kaplunovsky and J.~Louis,
%``Model independent analysis of soft terms in effective supergravity and in string theory,''
Phys. Lett. B \textbf{306}, 269-275 (1993)
doi:10.1016/0370-2693(93)90078-V
[arXiv:hep-th/9303040 [hep-th]].
%726 citations counted in INSPIRE as of 19 May 2022

%\cite{Louis:1994ht}
\bibitem{Louis:1994ht}
J.~Louis and Y.~Nir,
%``Some phenomenological implications of string loop effects,''
Nucl. Phys. B \textbf{447}, 18-34 (1995)
doi:10.1016/0550-3213(95)00155-L
[arXiv:hep-ph/9411429 [hep-ph]].
%58 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Choi:1997cm}
\bibitem{Choi:1997cm}
K.~Choi, H.~B.~Kim and C.~Munoz,
%``Four-dimensional effective supergravity and soft terms in M theory,''
Phys. Rev. D \textbf{57}, 7521-7528 (1998)
doi:10.1103/PhysRevD.57.7521
[arXiv:hep-th/9711158 [hep-th]].
%109 citations counted in INSPIRE as of 17 May 2022

%\cite{Brignole:1998dxa}
\bibitem{Brignole:1998dxa}
A.~Brignole, L.~E.~Ibanez and C.~Munoz,
%``Soft supersymmetry breaking terms from supergravity and superstring models,''
Adv. Ser. Direct. High Energy Phys. \textbf{18}, 125-148 (1998)
doi:10.1142/9789812839657\_0003
[arXiv:hep-ph/9707209 [hep-ph]].
%362 citations counted in INSPIRE as of 17 May 2022

%\cite{hep-th/9810155}
\bibitem{hep-th/9810155}
L.~Randall and R.~Sundrum,
%``Out of this world supersymmetry breaking,''
Nucl. Phys. B \textbf{557}, 79-118 (1999)
doi:10.1016/S0550-3213(99)00359-4
[arXiv:hep-th/9810155 [hep-th]].
%1893 citations counted in INSPIRE as of 19 May 2022

%\cite{hep-ph/9810442}
\bibitem{hep-ph/9810442}
G.~F.~Giudice, M.~A.~Luty, H.~Murayama and R.~Rattazzi,
%``Gaugino mass without singlets,''
JHEP \textbf{12}, 027 (1998)
doi:10.1088/1126-6708/1998/12/027
[arXiv:hep-ph/9810442 [hep-ph]].
%1538 citations counted in INSPIRE as of 19 May 2022

%\cite{hep-th/9911029}
\bibitem{hep-th/9911029}
J.~A.~Bagger, T.~Moroi and E.~Poppitz,
%``Anomaly mediation in supergravity theories,''
JHEP \textbf{04}, 009 (2000)
doi:10.1088/1126-6708/2000/04/009
[arXiv:hep-th/9911029 [hep-th]].
%354 citations counted in INSPIRE as of 19 May 2022

%\cite{hep-ph/0011081}
\bibitem{hep-ph/0011081}
P.~Binetruy, M.~K.~Gaillard and B.~D.~Nelson,
%``One loop soft supersymmetry breaking terms in superstring effective theories,''
Nucl. Phys. B \textbf{604}, 32-74 (2001)
doi:10.1016/S0550-3213(00)00759-8
[arXiv:hep-ph/0011081 [hep-ph]].
%143 citations counted in INSPIRE as of 19 May 2022

%\cite{Headrick:2005ch}
\bibitem{Headrick:2005ch}
M.~Headrick and T.~Wiseman,
%``Numerical Ricci-flat metrics on K3,''
Class. Quant. Grav. \textbf{22}, 4931-4960 (2005)
doi:10.1088/0264-9381/22/23/002
[arXiv:hep-th/0506129 [hep-th]].
%61 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Douglas:2006rr}
\bibitem{Douglas:2006rr}
M.~R.~Douglas, R.~L.~Karp, S.~Lukic and R.~Reinbacher,
%``Numerical Calabi-Yau metrics,''
J. Math. Phys. \textbf{49}, 032302 (2008)
doi:10.1063/1.2888403
[arXiv:hep-th/0612075 [hep-th]].
%59 citations counted in INSPIRE as of 14 May 2022

%\cite{Braun:2007sn}
\bibitem{Braun:2007sn}
V.~Braun, T.~Brelidze, M.~R.~Douglas and B.~A.~Ovrut,
%``Calabi-Yau Metrics for Quotients and Complete Intersections,''
JHEP \textbf{05}, 080 (2008)
doi:10.1088/1126-6708/2008/05/080
[arXiv:0712.3563 [hep-th]].
%54 citations counted in INSPIRE as of 14 May 2022

%\cite{Headrick:2009jz}
\bibitem{Headrick:2009jz}
M.~Headrick and A.~Nassar,
%``Energy functionals for Calabi-Yau metrics,''
Adv. Theor. Math. Phys. \textbf{17}, no.5, 867-902 (2013)
doi:10.4310/ATMP.2013.v17.n5.a1
[arXiv:0908.2635 [hep-th]].
%38 citations counted in INSPIRE as of 14 May 2022

%\cite{Douglas:2006hz}
\bibitem{Douglas:2006hz}
M.~R.~Douglas, R.~L.~Karp, S.~Lukic and R.~Reinbacher,
%``Numerical solution to the hermitian Yang-Mills equation on the Fermat quintic,''
JHEP \textbf{12}, 083 (2007)
doi:10.1088/1126-6708/2007/12/083
[arXiv:hep-th/0606261 [hep-th]].
%51 citations counted in INSPIRE as of 14 May 2022

%\cite{Anderson:2011ed}
\bibitem{Anderson:2011ed}
L.~B.~Anderson, V.~Braun and B.~A.~Ovrut,
%``Numerical Hermitian Yang-Mills Connections and Kahler Cone Substructure,''
JHEP \textbf{01}, 014 (2012)
doi:10.1007/JHEP01(2012)014
[arXiv:1103.3041 [hep-th]].
%24 citations counted in INSPIRE as of 14 May 2022

%\cite{Anderson:2010ke}
\bibitem{Anderson:2010ke}
L.~B.~Anderson, V.~Braun, R.~L.~Karp and B.~A.~Ovrut,
%``Numerical Hermitian Yang-Mills Connections and Vector Bundle Stability in Heterotic Theories,''
JHEP \textbf{06}, 107 (2010)
doi:10.1007/JHEP06(2010)107
[arXiv:1004.4399 [hep-th]].
%35 citations counted in INSPIRE as of 14 May 2022

%\cite{Cui:2019uhy}
\bibitem{Cui:2019uhy}
W.~Cui and J.~Gray,
%``Numerical Metrics, Curvature Expansions and Calabi-Yau Manifolds,''
JHEP \textbf{05}, 044 (2020)
doi:10.1007/JHEP05(2020)044
[arXiv:1912.11068 [hep-th]].
%14 citations counted in INSPIRE as of 14 May 2022

%\cite{Anderson:2020hux}
\bibitem{Anderson:2020hux}
L.~B.~Anderson, M.~Gerdes, J.~Gray, S.~Krippendorf, N.~Raghuram and F.~Ruehle,
%``Moduli-dependent Calabi-Yau and SU(3)-structure metrics from Machine Learning,''
JHEP \textbf{05}, 013 (2021)
doi:10.1007/JHEP05(2021)013
[arXiv:2012.04656 [hep-th]].
%34 citations counted in INSPIRE as of 19 May 2022

%\cite{Douglas:2020hpv}
\bibitem{Douglas:2020hpv}
M.~R.~Douglas, S.~Lakshminarasimhan and Y.~Qi,
%``Numerical Calabi-Yau metrics from holomorphic networks,''
[arXiv:2012.04797 [hep-th]].
%28 citations counted in INSPIRE as of 14 May 2022

%\cite{Keller:2009vj}
\bibitem{Keller:2009vj}
J.~Keller and S.~Lukic,
%``Numerical Weil\textendash{}Petersson metrics on moduli spaces of Calabi\textendash{}Yau manifolds,''
J. Geom. Phys. \textbf{92}, 252-270 (2015)
doi:10.1016/j.geomphys.2015.02.018
[arXiv:0907.1387 [math.DG]].
%9 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Braun:2008jp}
\bibitem{Braun:2008jp}
V.~Braun, T.~Brelidze, M.~R.~Douglas and B.~A.~Ovrut,
%``Eigenvalues and Eigenfunctions of the Scalar Laplace Operator on Calabi-Yau Manifolds,''
JHEP \textbf{07}, 120 (2008)
doi:10.1088/1126-6708/2008/07/120
[arXiv:0805.3689 [hep-th]].
%46 citations counted in INSPIRE as of 14 May 2022

%\cite{Ashmore:2020ujw}
\bibitem{Ashmore:2020ujw}
A.~Ashmore,
%``Eigenvalues and eigenforms on Calabi-Yau threefolds,''
[arXiv:2011.13929 [hep-th]].
%10 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Deen:2016zfr}
\bibitem{Deen:2016zfr}
R.~Deen, B.~A.~Ovrut and A.~Purves,
%``Supersymmetric Sneutrino-Higgs Inflation,''
Phys. Lett. B \textbf{762}, 441-446 (2016)
doi:10.1016/j.physletb.2016.09.059
[arXiv:1606.00431 [hep-ph]].
%16 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Martin:1997ns}
\bibitem{Martin:1997ns}
S.~P.~Martin,
%``A Supersymmetry primer,''
Adv. Ser. Direct. High Energy Phys. \textbf{18}, 1-98 (1998)
doi:10.1142/9789812839657\_0001
[arXiv:hep-ph/9709356 [hep-ph]].
%4449 citations counted in INSPIRE as of 23 May 2022

%\cite{Fundira:2017vip}
\bibitem{Fundira:2017vip}
P.~Fundira and A.~Purves,
%``Bayesian naturalness, simplicity, and testability applied to the $B−L$ MSSM GUT,''
Int. J. Mod. Phys. A \textbf{33}, no.11, 1841004 (2018)
doi:10.1142/S0217751X1841004X
[arXiv:1708.07835 [hep-ph]].
%10 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Senjanovic:1975rk}
\bibitem{Senjanovic:1975rk}
G.~Senjanovic and R.~N.~Mohapatra,
%``Exact Left-Right Symmetry and Spontaneous Violation of Parity,''
Phys. Rev. D \textbf{12}, 1502 (1975)
doi:10.1103/PhysRevD.12.1502
%2310 citations counted in INSPIRE as of 22 May 2022

%\cite{Grimus:1993fx}
\bibitem{Grimus:1993fx}
W.~Grimus,
%``Introduction to left-right symmetric models,''
UWTHPH-1993-10.
%0 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Mukhopadhyaya:1998xj}
\bibitem{Mukhopadhyaya:1998xj}
B.~Mukhopadhyaya, S.~Roy and F.~Vissani,
%``Correlation between neutrino oscillations and collider signals of supersymmetry in an R-parity violating model,''
Phys. Lett. B \textbf{443}, 191-195 (1998)
doi:10.1016/S0370-2693(98)01288-X
[arXiv:hep-ph/9808265 [hep-ph]].
%185 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Chun:1998ub}
\bibitem{Chun:1998ub}
E.~J.~Chun and J.~S.~Lee,
%``Implication of Super-Kamiokande data on R-parity violation,''
Phys. Rev. D \textbf{60}, 075006 (1999)
doi:10.1103/PhysRevD.60.075006
[arXiv:hep-ph/9811201 [hep-ph]].
%71 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Chun:1999bq}
\bibitem{Chun:1999bq}
E.~J.~Chun and S.~K.~Kang,
%``One loop corrected neutrino masses and mixing in supersymmetric standard model without R-parity,''
Phys. Rev. D \textbf{61}, 075012 (2000)
doi:10.1103/PhysRevD.61.075012
[arXiv:hep-ph/9909429 [hep-ph]].
%101 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Hirsch:2000ef}
\bibitem{Hirsch:2000ef}
M.~Hirsch, M.~A.~Diaz, W.~Porod, J.~C.~Romao and J.~W.~F.~Valle,
%``Neutrino masses and mixings from supersymmetry with bilinear R parity violation: A Theory for solar and atmospheric neutrino oscillations,''
Phys. Rev. D \textbf{62}, 113008 (2000)
[erratum: Phys. Rev. D \textbf{65}, 119901 (2002)]
doi:10.1103/PhysRevD.62.113008
[arXiv:hep-ph/0004115 [hep-ph]].
%393 citations counted in INSPIRE as of 25 Apr 2022

%\cite{FileviezPerez:2008sx}
\bibitem{FileviezPerez:2008sx}
P.~Fileviez Perez and S.~Spinner,
%``Spontaneous R-Parity Breaking and Left-Right Symmetry,''
Phys. Lett. B \textbf{673}, 251-254 (2009)
doi:10.1016/j.physletb.2009.02.047
[arXiv:0811.3424 [hep-ph]].
%93 citations counted in INSPIRE as of 10 May 2022

%\cite{Everett:2009vy}
\bibitem{Everett:2009vy}
L.~L.~Everett, P.~Fileviez Perez and S.~Spinner,
%``The Right Side of Tev Scale Spontaneous R-Parity Violation,''
Phys. Rev. D \textbf{80}, 055007 (2009)
doi:10.1103/PhysRevD.80.055007
[arXiv:0906.4095 [hep-ph]].
%36 citations counted in INSPIRE as of 10 May 2022

%\cite{Perez:2013kla}
\bibitem{Perez:2013kla}
P.~Fileviez Perez and S.~Spinner,
%``Supersymmetry at the LHC and The Theory of R-parity,''
Phys. Lett. B \textbf{728}, 489-495 (2014)
doi:10.1016/j.physletb.2013.12.022
[arXiv:1308.0524 [hep-ph]].
%33 citations counted in INSPIRE as of 10 May 2022

%\cite{Ghosh:2010hy}
\bibitem{Ghosh:2010hy}
D.~K.~Ghosh, G.~Senjanovic and Y.~Zhang,
%``Naturally Light Sterile Neutrinos from Theory of R-parity,''
Phys. Lett. B \textbf{698}, 420-424 (2011)
doi:10.1016/j.physletb.2011.03.039
[arXiv:1010.3968 [hep-ph]].
%50 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Barger:2010iv}
\bibitem{Barger:2010iv}
V.~Barger, P.~Fileviez Perez and S.~Spinner,
%``Three Layers of Neutrinos,''
Phys. Lett. B \textbf{696}, 509-512 (2011)
doi:10.1016/j.physletb.2011.01.015
[arXiv:1010.4023 [hep-ph]].
%46 citations counted in INSPIRE as of 10 May 2022

%\cite{Mohapatra:1986aw}
\bibitem{Mohapatra:1986aw}
R.~N.~Mohapatra,
%``Mechanism for Understanding Small Neutrino Mass in Superstring Theories,''
Phys. Rev. Lett. \textbf{56}, 561-563 (1986)
doi:10.1103/PhysRevLett.56.561
%593 citations counted in INSPIRE as of 19 May 2022

%\cite{ATLAS:2014fka}
\bibitem{ATLAS:2014fka}
G.~Aad \textit{et al.} [ATLAS],
%``Searches for heavy long-lived charged particles with the ATLAS detector in proton-proton collisions at $ \sqrt{s}=8 $ TeV,''
JHEP \textbf{01}, 068 (2015)
doi:10.1007/JHEP01(2015)068
[arXiv:1411.6795 [hep-ex]].
%153 citations counted in INSPIRE as of 12 May 2022

%\cite{Aad:2015rba}
\bibitem{Aad:2015rba}
G.~Aad \textit{et al.} [ATLAS],
%``Search for massive, long-lived particles using multitrack displaced vertices or displaced lepton pairs in pp collisions at $\sqrt{s}$ = 8 TeV with the ATLAS detector,''
Phys. Rev. D \textbf{92}, no.7, 072004 (2015)
doi:10.1103/PhysRevD.92.072004
[arXiv:1504.05162 [hep-ex]].
%208 citations counted in INSPIRE as of 17 May 2022

%\cite{Capozzi:2018ubv}
\bibitem{Capozzi:2018ubv}
F.~Capozzi, E.~Lisi, A.~Marrone and A.~Palazzo,
%``Current unknowns in the three neutrino framework,''
Prog. Part. Nucl. Phys. \textbf{102}, 48-72 (2018)
doi:10.1016/j.ppnp.2018.05.005
[arXiv:1804.09678 [hep-ph]].
%226 citations counted in INSPIRE as of 20 May 2022

%\cite{Barbier:2004ez}
\bibitem{Barbier:2004ez}
R.~Barbier, C.~Berat, M.~Besancon, M.~Chemtob, A.~Deandrea, E.~Dudas, P.~Fayet, S.~Lavignac, G.~Moreau and E.~Perez, \textit{et al.}
%``R-parity violating supersymmetry,''
Phys. Rept. \textbf{420}, 1-202 (2005)
doi:10.1016/j.physrep.2005.08.006
[arXiv:hep-ph/0406039 [hep-ph]].
%1272 citations counted in INSPIRE as of 23 May 2022

%\cite{Aaboud:2017buh}
\bibitem{Aaboud:2017buh}
M.~Aaboud \textit{et al.} [ATLAS],
%``Search for new high-mass phenomena in the dilepton final state using 36 fb$^{−1}$ of proton-proton collision data at $ \sqrt{s}=13 $ TeV with the ATLAS detector,''
JHEP \textbf{10}, 182 (2017)
doi:10.1007/JHEP10(2017)182
[arXiv:1707.02424 [hep-ex]].
%415 citations counted in INSPIRE as of 20 May 2022

%\cite{Aaboud:2018wps}
\bibitem{Aaboud:2018wps}
M.~Aaboud \textit{et al.} [ATLAS],
%``Measurement of the Higgs boson mass in the $H\rightarrow ZZ^* \rightarrow 4\ell$ and $H \rightarrow \gamma\gamma$ channels with $\sqrt{s}=13$ TeV $pp$ collisions using the ATLAS detector,''
Phys. Lett. B \textbf{784}, 345-366 (2018)
doi:10.1016/j.physletb.2018.07.050
[arXiv:1806.00242 [hep-ex]].
%181 citations counted in INSPIRE as of 17 May 2022

%\cite{ATLAS:2015jla}
\bibitem{ATLAS:2015jla}
 [ATLAS],
%``A search for $B-L$ $R$-Parity violating scalar top decays in $\sqrt{s} = 8$ TeV $pp$ collisions with the ATLAS experiment,''
ATLAS-CONF-2015-015.
%21 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Jackson:2015lmj}
\bibitem{Jackson:2015lmj}
B.~Jackson,
%``A Search For $B-L$ $R$-Parity-Violating Scalar Top Decays in $\sqrt{s} = 8$ TeV $pp$ Collisions With The ATLAS Experiment,''
CERN-THESIS-2015-129.
%2 citations counted in INSPIRE as of 25 Apr 2022

%\cite{ATLAS:2017hbw}
\bibitem{ATLAS:2017hbw}
 [ATLAS],
%``A search for $B-L$ $R$-parity-violating scalar tops in $\sqrt{s}$ = 13 TeV $pp$ collisions with the ATLAS experiment,''
ATLAS-CONF-2017-036.
%10 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Aaboud:2017opj}
\bibitem{Aaboud:2017opj}
M.~Aaboud \textit{et al.} [ATLAS],
%``Search for B-L R -parity-violating top squarks in $\sqrt s$ =13  TeV pp collisions with the ATLAS experiment,''
Phys. Rev. D \textbf{97}, no.3, 032003 (2018)
doi:10.1103/PhysRevD.97.032003
[arXiv:1710.05544 [hep-ex]].
%38 citations counted in INSPIRE as of 16 May 2022

%\cite{Paige:2003mg}
\bibitem{Paige:2003mg}
F.~E.~Paige, S.~D.~Protopopescu, H.~Baer and X.~Tata,
%``ISAJET 7.69: A Monte Carlo event generator for pp, anti-p p, and e+e- reactions,''
[arXiv:hep-ph/0312045 [hep-ph]].
%791 citations counted in INSPIRE as of 05 May 2022

%\cite{Athron:2014yba}
\bibitem{Athron:2014yba}
P.~Athron, J.~h.~Park, D.~St\"ockinger and A.~Voigt,
%``FlexibleSUSY\textemdash{}A spectrum generator generator for supersymmetric models,''
Comput. Phys. Commun. \textbf{190}, 139-172 (2015)
doi:10.1016/j.cpc.2014.12.020
[arXiv:1406.2319 [hep-ph]].
%146 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Ellwanger:2006rn}
\bibitem{Ellwanger:2006rn}
U.~Ellwanger and C.~Hugonie,
%``NMSPEC: A Fortran code for the sparticle and Higgs masses in the NMSSM with GUT scale boundary conditions,''
Comput. Phys. Commun. \textbf{177}, 399-407 (2007)
doi:10.1016/j.cpc.2007.05.001
[arXiv:hep-ph/0612134 [hep-ph]].
%203 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Djouadi:2002ze}
\bibitem{Djouadi:2002ze}
A.~Djouadi, J.~L.~Kneur and G.~Moultaka,
%``SuSpect: A Fortran code for the supersymmetric and Higgs particle spectrum in the MSSM,''
Comput. Phys. Commun. \textbf{176}, 426-455 (2007)
doi:10.1016/j.cpc.2006.11.009
[arXiv:hep-ph/0211331 [hep-ph]].
%1073 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Staub:2008uz}
\bibitem{Staub:2008uz}
F.~Staub,
%``SARAH,''
[arXiv:0806.0538 [hep-ph]].
%411 citations counted in INSPIRE as of 13 May 2022

%\cite{Porod:2003um}
\bibitem{Porod:2003um}
W.~Porod,
%``SPheno, a program for calculating supersymmetric spectra, SUSY particle decays and SUSY particle production at e+ e- colliders,''
Comput. Phys. Commun. \textbf{153}, 275-315 (2003)
doi:10.1016/S0010-4655(03)00222-4
[arXiv:hep-ph/0301101 [hep-ph]].
%1102 citations counted in INSPIRE as of 13 May 2022

%\cite{Chowdhury:2011zr}
\bibitem{Chowdhury:2011zr}
D.~Chowdhury, R.~Garani and S.~K.~Vempati,
%``SUSEFLAV: Program for supersymmetric mass spectra with seesaw mechanism and rare lepton flavor violating decays,''
Comput. Phys. Commun. \textbf{184}, 899-918 (2013)
doi:10.1016/j.cpc.2012.10.031
[arXiv:1109.3551 [hep-ph]].
%43 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Allanach:2016rxd}
\bibitem{Allanach:2016rxd}
B.~C.~Allanach, S.~P.~Martin, D.~G.~Robertson and R.~Ruiz de Austri,
%``The Inclusion of Two-Loop SUSYQCD Corrections to Gluino and Squark Pole Masses in the Minimal and Next-to-Minimal Supersymmetric Standard Model: SOFTSUSY3.7,''
Comput. Phys. Commun. \textbf{219}, 339-345 (2017)
doi:10.1016/j.cpc.2017.05.006
[arXiv:1601.06657 [hep-ph]].
%20 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Mohapatra:2015fua}
\bibitem{Mohapatra:2015fua}
R.~N.~Mohapatra,
%``Supersymmetry and R-parity: an Overview,''
Phys. Scripta \textbf{90}, 088004 (2015)
doi:10.1088/0031-8949/90/8/088004
[arXiv:1503.06478 [hep-ph]].
%39 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Dercks:2017lfq}
\bibitem{Dercks:2017lfq}
D.~Dercks, H.~Dreiner, M.~E.~Krauss, T.~Opferkuch and A.~Reinert,
%``R-Parity Violation at the LHC,''
Eur. Phys. J. C \textbf{77}, no.12, 856 (2017)
doi:10.1140/epjc/s10052-017-5414-4
[arXiv:1706.09418 [hep-ph]].
%32 citations counted in INSPIRE as of 18 May 2022

%\cite{Hirsch:2008ur}
\bibitem{Hirsch:2008ur}
M.~Hirsch, A.~Vicente and W.~Porod,
%``Spontaneous R-parity violation: Lightest neutralino decays and neutrino mixing angles at future colliders,''
Phys. Rev. D \textbf{77}, 075005 (2008)
doi:10.1103/PhysRevD.77.075005
[arXiv:0802.2896 [hep-ph]].
%27 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Mitsou:2015eka}
\bibitem{Mitsou:2015eka}
V.~A.~Mitsou,
%``Exploring neutrino physics at LHC via R-parity violating SUSY,''
J. Phys. Conf. Ser. \textbf{631}, no.1, 012074 (2015)
doi:10.1088/1742-6596/631/1/012074
[arXiv:1502.07997 [hep-ph]].
%6 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Mitsou:2015kpa}
\bibitem{Mitsou:2015kpa}
V.~A.~Mitsou,
%``R-parity violating supersymmetry and neutrino physics: experimental signatures,''
PoS \textbf{PLANCK2015}, 085 (2015)
doi:10.22323/1.258.0085
[arXiv:1510.02660 [hep-ph]].
%9 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Bomark:2014rra}
\bibitem{Bomark:2014rra}
N.~E.~Bomark, A.~Kvellestad, S.~Lola, P.~Osland and A.~R.~Raklev,
%``R-parity violating chargino decays at the LHC,''
JHEP \textbf{12}, 121 (2014)
doi:10.1007/JHEP12(2014)121
[arXiv:1410.0921 [hep-ph]].
%6 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Csaki:2015uza}
\bibitem{Csaki:2015uza}
C.~Csaki, E.~Kuflik, S.~Lombardo, O.~Slone and T.~Volansky,
%``Phenomenology of a Long-Lived LSP with R-Parity Violation,''
JHEP \textbf{08}, 016 (2015)
doi:10.1007/JHEP08(2015)016
[arXiv:1505.00784 [hep-ph]].
%54 citations counted in INSPIRE as of 12 May 2022

%\cite{Athron:2017fxj}
\bibitem{Athron:2017fxj}
P.~Athron, C.~Balazs, B.~Farmer, A.~Fowlie, D.~Harries and D.~Kim,
%``Bayesian analysis and naturalness of (Next-to-)Minimal Supersymmetric Models,''
JHEP \textbf{10}, 160 (2017)
doi:10.1007/JHEP10(2017)160
[arXiv:1709.07895 [hep-ph]].
%18 citations counted in INSPIRE as of 03 May 2022

%\cite{Fichet:2012sn}
\bibitem{Fichet:2012sn}
S.~Fichet,
%``Quantified naturalness from Bayesian statistics,''
Phys. Rev. D \textbf{86}, 125029 (2012)
doi:10.1103/PhysRevD.86.125029
[arXiv:1204.4940 [hep-ph]].
%60 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Gherghetta:1999sw}
\bibitem{Gherghetta:1999sw}
T.~Gherghetta, G.~F.~Giudice and J.~D.~Wells,
%``Phenomenological consequences of supersymmetry with anomaly induced masses,''
Nucl. Phys. B \textbf{559}, 27-47 (1999)
doi:10.1016/S0550-3213(99)00429-0
[arXiv:hep-ph/9904378 [hep-ph]].
%455 citations counted in INSPIRE as of 11 May 2022

%\cite{Cheng:1998hc}
\bibitem{Cheng:1998hc}
H.~C.~Cheng, B.~A.~Dobrescu and K.~T.~Matchev,
%``Generic and chiral extensions of the supersymmetric standard model,''
Nucl. Phys. B \textbf{543}, 47-72 (1999)
doi:10.1016/S0550-3213(99)00012-7
[arXiv:hep-ph/9811316 [hep-ph]].
%142 citations counted in INSPIRE as of 11 May 2022

%\cite{Ibe:2012sx}
\bibitem{Ibe:2012sx}
M.~Ibe, S.~Matsumoto and R.~Sato,
%``Mass Splitting between Charged and Neutral Winos at Two-Loop Level,''
Phys. Lett. B \textbf{721}, 252-260 (2013)
doi:10.1016/j.physletb.2013.03.015
[arXiv:1212.5989 [hep-ph]].
%161 citations counted in INSPIRE as of 05 May 2022

%\cite{Aaboud:2017iio}
\bibitem{Aaboud:2017iio}
M.~Aaboud \textit{et al.} [ATLAS],
%``Search for long-lived, massive particles in events with displaced vertices and missing transverse momentum in $\sqrt{s}$ = 13 TeV $pp$ collisions with the ATLAS detector,''
Phys. Rev. D \textbf{97}, no.5, 052012 (2018)
doi:10.1103/PhysRevD.97.052012
[arXiv:1710.04901 [hep-ex]].
%170 citations counted in INSPIRE as of 17 May 2022

%\cite{Sirunyan:2018vlw}
\bibitem{Sirunyan:2018vlw}
A.~M.~Sirunyan \textit{et al.} [CMS],
%``Search for long-lived particles decaying into displaced jets in proton-proton collisions at $\sqrt{s}=$ 13 TeV,''
Phys. Rev. D \textbf{99}, no.3, 032011 (2019)
doi:10.1103/PhysRevD.99.032011
[arXiv:1811.07991 [hep-ex]].
%57 citations counted in INSPIRE as of 23 May 2022

%\cite{CMS:2014hka}
\bibitem{CMS:2014hka}
V.~Khachatryan \textit{et al.} [CMS],
%``Search for long-lived particles that decay into final states containing two electrons or two muons in proton-proton collisions at $\sqrt{s} =$ 8 TeV,''
Phys. Rev. D \textbf{91}, no.5, 052012 (2015)
doi:10.1103/PhysRevD.91.052012
[arXiv:1411.6977 [hep-ex]].
%139 citations counted in INSPIRE as of 19 May 2022

%\cite{Aaboud:2018aqj}
\bibitem{Aaboud:2018aqj}
M.~Aaboud \textit{et al.} [ATLAS],
%``Search for long-lived particles produced in $pp$ collisions at $\sqrt{s}=13$  TeV that decay into displaced hadronic jets in the ATLAS muon spectrometer,''
Phys. Rev. D \textbf{99}, no.5, 052005 (2019)
doi:10.1103/PhysRevD.99.052005
[arXiv:1811.07370 [hep-ex]].
%84 citations counted in INSPIRE as of 17 May 2022

%\cite{ATLAS-CONF-2018-003}
\bibitem{ATLAS-CONF-2018-003}
 [ATLAS],
%``Reinterpretation of searches for supersymmetry in models with variable $R$-parity-violating coupling strength and long-lived $R$-hadrons,''
ATLAS-CONF-2018-003.
%23 citations counted in INSPIRE as of 25 Apr 2022

%\cite{Chou:2016lxi}
\bibitem{Chou:2016lxi}
J.~P.~Chou, D.~Curtin and H.~J.~Lubatti,
%``New Detectors to Explore the Lifetime Frontier,''
Phys. Lett. B \textbf{767}, 29-36 (2017)
doi:10.1016/j.physletb.2017.01.043
[arXiv:1606.06298 [hep-ph]].
%202 citations counted in INSPIRE as of 23 May 2022

%\cite{deFlorian:2016spz}
\bibitem{deFlorian:2016spz}
D.~de Florian \textit{et al.} [LHC Higgs Cross Section Working Group],
%``Handbook of LHC Higgs Cross Sections: 4. Deciphering the Nature of the Higgs Sector,''
doi:10.23731/CYRM-2017-002
[arXiv:1610.07922 [hep-ph]].
%1646 citations counted in INSPIRE as of 23 May 2022

%\cite{Dine:1987gj}
\bibitem{Dine:1987gj}
M.~Dine, I.~Ichinose and N.~Seiberg,
%``F Terms and d Terms in String Theory,''
Nucl. Phys. B \textbf{293}, 253-265 (1987)
doi:10.1016/0550-3213(87)90072-1
%440 citations counted in INSPIRE as of 29 Apr 2022

%\cite{Anastasopoulos:2006cz}
\bibitem{Anastasopoulos:2006cz}
P.~Anastasopoulos, M.~Bianchi, E.~Dudas and E.~Kiritsis,
%``Anomalies, anomalous U(1)'s and generalized Chern-Simons terms,''
JHEP \textbf{11}, 057 (2006)
doi:10.1088/1126-6708/2006/11/057
[arXiv:hep-th/0605225 [hep-th]].
%190 citations counted in INSPIRE as of 06 May 2022

%\cite{Blumenhagen:2006ux}
\bibitem{Blumenhagen:2006ux}
R.~Blumenhagen, S.~Moster and T.~Weigand,
%``Heterotic GUT and standard model vacua from simply connected Calabi-Yau manifolds,''
Nucl. Phys. B \textbf{751}, 186-221 (2006)
doi:10.1016/j.nuclphysb.2006.06.005
[arXiv:hep-th/0603015 [hep-th]].
%176 citations counted in INSPIRE as of 14 May 2022

%\cite{Ibanez:2012zz}
\bibitem{Ibanez:2012zz}
L.~E.~Ibanez and A.~M.~Uranga,
%``String theory and particle physics: An introduction to string phenomenology,''
%51 citations counted in INSPIRE as of 05 May 2022

%\cite{Shifman:2012zz}
\bibitem{Shifman:2012zz}
M.~Shifman,
%``Advanced topics in quantum field theory.: A lecture course,''
%18 citations counted in INSPIRE as of 23 May 2022
